Cloud Property Graph: Connecting Cloud Security Assessments with Static Code Analysis

In this paper, we present the Cloud Property Graph (CloudPG), which bridges the gap between static code analysis and runtime security assessment of cloud services. The CloudPG is able to resolve data flows between cloud applications deployed on different resources, and contextualizes the graph with runtime information, such as encryption settings. To provide a vendor- and technology-independent representation of a cloud service's security posture, the graph is based on an ontology of cloud resources, their functionalities and security features. We show, using an example, that our CloudPG framework can be used by security experts to identify weaknesses in their cloud deployments, spanning multiple vendors or technologies, such as AWS, Azure and Kubernetes. This includes misconfigurations, such as publicly accessible storages or undesired data flows within a cloud service, as restricted by regulations such as GDPR.

==> sections/background.tex <==
%!TEX root = ../cloudpg.tex

\subsection{Graph-based Static Code Analysis}

%In a typical cloud environment, multiple source code projects are combined as micro-services and interact with each
%other. This requires an analysis method that scales with code size and/or number of projects especially when they are
%combined into one representation \todo{consolidate naming: what is a project, service, representation, and what does the
%code size have to do with that?}. 
Yamaguchi et al. first introduced the concept of a Code Property Graph (CPG)~\cite{yamaguchi2014modeling}, a directed
attributed graph representing source code that allows the analysis of large source code projects. The CPG is a graph of
nodes that represent the syntactic elements of the source code and edges that put them into relation. The type of edges
of the same type are used to represent different aspects of source code:
\begin{itemize}
	\item the program's syntactic structure, in the form of an Abstract Syntax Tree (AST),
	\item the program's execution order, as Control Flow Graph (CFG) between the AST-nodes,
	\item and the program's data flow, in a Data Flow Graph (DFG) or Program Dependence Graph (PDG).
\end{itemize}

The representation of source code in a CPG allows to search large code bases for vulnerabilities and patterns that can
give insight on whether a program behaves in accordance to some compliance criterion. A CPG is constructed from source
code or an intermediate representation, stored in a graph-database and can then be queried with declarative
languages such as Cypher. CPG-based analysis methods, in contrast to Symbolic Execution or
Model Checking, do not simulate representations of program state, but perform searches on structural information
augmented with abstracted graphs of behavior. This results in trading accuracy for more efficiency and avoid state
explosion problems that other methods are susceptible to when analyzing modern code bases that are large in size.

Several implementations of building CPGs from application code exist that differ in the abstraction level and the
languages that they support. \textit{Plume}\footnote{\url{https://github.com/plume-oss/plume}} and
\textit{Graft}\footnote{\url{https://github.com/wimkeir/graft}} take Java bytecode.
\textit{Joern}\footnote{\url{https://github.com/ShiftLeftSecurity/codepropertygraph}} is a platform for robust analysis
of C/C++ code that also supports other languages, including Java when provided in its bytecode format. The
\textit{cpg}\footnote{\url{https://github.com/Fraunhofer-AISEC/cpg}} project represents control flow on a finer
granularity, also capturing the order in which expressions are evaluated. The library can represent Java, C/C++ as well
as Python and Go source code in a unified format, allowing the analysis of a heterogeneous cloud service, written in multiple
languages.

\subsection{Ontology Modelling}
\label{background:ontology_modelling}
In Section \ref{ontology} we propose an ontology for cloud resources and their security properties. 
% In fact, this ontology is composed of three interrelated taxonomies: a generalized cloud resource taxonomy, a software framework taxonomy, and an abstract security property taxonomy. Also it is instantiated with concrete resources of Microsoft Azure, Amazon Web Services and the Kubernetes technology stack.
In our ontology, we make use of the Web Ontology Language (OWL) \cite{bechhofer2004owl} which is the
de-facto standard for modeling the semantics of web-based resources. % https://www.w3.org/2001/sw/wiki/OWL
Its main constructs are \textit{classes} and \textit{properties}. Furthermore, \textit{instances} can be defined which represent concrete individuals of a certain class, e.g., an AWS S3 Bucket is an instance of the ObjectStorage class.

% The basic concept within OWL is an \textit{Entity}, which is used to define the vocabulary terms within an Ontology.
% They are further structured in several concepts, such as classes or (named) individuals. According to the OWL
% specification, a named individual represents actual objects from the modeled domain, e.g., the Cloud ecosystem. In our
% case, we use named individuals to represent actual Cloud offerings by vendors, such as Amazon Web Services. A class in
% OWL represents a set of individuals.

All entities can also have a set of properties. \textit{Data and object properties} can be used
to describe relationships between entities within the ontology. Additionally, \textit{annotation properties} can
be used to describe certain meta-information about the entity. It is important to understand that properties in OWL are
not just literal strings but are entities themselves, providing a uniform way to represent certain semantic information
such as the name or the inheritance of entities across the ontology.


==> sections/requirements.tex <==
%!TEX root = ../cloudpg.tex

% TODO: stays in, but needs to be shortened a little bit

With our contributions we want to enable security analysts to contextualize the security posture of code deployed on
cloud resources. Therefore, we define the following design goals, which guide the architecture design in
Section~\ref{approach} as well as the implementation in Section~\ref{implementation}. Lastly, we evaluate our design
goals in Section~\ref{sec:discussion}.

\newenvironment{requirement}{\begin{enumerate}[label=\textbf{D\arabic*}]\raggedright}{\end{enumerate}}

\begin{requirement}
	\item\label{dg:abstraction} \textbf{Analyze cloud-hosted code independently of the resource type or cloud provider:}
		the security analysis of deployments should be executable across cloud resources and cloud providers. The
		CloudPG aims to offer a service-independent representation of resources in the Cloud. %This is especially
	%relevant for cloud resources which offer additional security guarantees, such as encryption. Using a generic
	%representation of their configuration across all resources can help to identify weaknesses more easily.

	\item\label{dg:bridge} \textbf{Bridge the gap between static code analysis and runtime assessment:} Methods of
	static code analysis need to be enhanced with an analysis of the deployment context, e.g. the configuration of the
	virtual machine where an application is deployed to.
	%needs to be enhanced with an analysis of its deployment context
	%often developers
	%make assumptions about the deployment environment an application is running on and therefore choose not to deal with
	%specific security properties, such as authentication or encryption as part of the application code. Static code
	%analysis alone cannot sufficiently evaluate the security posture of cloud-deployed code. This analysis therefore
	%needs to be enhanced with an analysis of its deployment context.

	\item\label{dg:dataflow}\textbf{Track end-to-end data flows across cloud resources:} a cloud system is typically
	composed of many resources interacting witch each other, e.g., chains of serverless functions. The security of
	cloud-hosted code therefore needs to be evaluated in context of the components it interacts with, for instance to
	identify storing secrets to publicly accessible storage locations.

	\item\label{dg:searchable}\textbf{Provide an efficiently searchable representation of the results:} to enable
	queries and future extensions enabling more sophisticated analysis, the results must be stored in a format that is
	efficiently searchable.
\end{requirement}

